Solving Large Sequential Games with the Excessive Gap Technique

There has been tremendous recent progress on equilibrium-finding algorithms for zero-sum imperfect-information extensive-form games, but there has been a puzzling gap between theory and practice. First-order methods have significantly better theoretical convergence rates than any counterfactual-regret minimization (CFR) variant. Despite this, CFR variants have been favored in practice. Experiments with first-order methods have only been conducted on small- and medium-sized games because those methods are complicated to implement in this setting, and because CFR variants have been enhanced extensively for over a decade they perform well in practice. In this paper we show that a particular first-order method, a state-of-the-art variant of the excessive gap technique---instantiated with the dilated entropy distance function---can efficiently solve large real-world problems competitively with CFR and its variants. We show this on large endgames encountered by the Libratus poker AI, which recently beat top human poker specialist professionals at no-limit Texas hold'em. We show experimental results on our variant of the excessive gap technique as well as a prior version. We introduce a numerically friendly implementation of the smoothed best response computation associated with first-order methods for extensive-form game solving. We present, to our knowledge, the first GPU implementation of a first-order method for extensive-form games. We present comparisons of several excessive gap technique and CFR variants.

==> text/cfr.tex <==
\section{Counterfactual Regret Minimization}

For CFR we consider several variants.\footnote{All variants use the alternating updates
scheme.} We run CFR with RM (CFR(RM)), {\rmp} (CFR({\rmp})), and {\cfrp} which is
CFR with {\rmp} and a linear averaging scheme. We now describe these variants. Detailed descriptions can also be found in \citet{Zinkevich07:Regret}
and \citet{Tammelin15:Solving}.


A generalized CFR description is given in Algorithm~\ref{alg:cfr}. It is
parameterized by a stepsize sequence $\{\alpha^t\}$, choices for simplex regret
minimizers $\textsc{R}_x,\textsc{R}_y$ for each player, and a convergence goal
$\epsilon$. At every iteration, the algorithm computes the gradient for the
$x$-player with respect to the previous iterate $y^{t-1}$, traverses the
simplexes $S_\cX$ in bottom-up order, and at every simplex updates the parent
gradient with the current value of the strategy at the simplex, and then updates
the simplex strategy via the regret minimizer $\textsc{R}_x$. Finally the same
sequence of steps is performed for the $y$-player, except that the current
iterate $x^t$ is used for computing the gradient (using $x^t$ rather than
$x^{t-1}$ to compute the gradient is called \emph{alternating updates} and
is used in most modern CFR implementations).
\begin{algorithm}[h!]
 \caption{\textsc{Gen-CFR}(stepsize sequence $\{\alpha^t\}$, regret minimizers
   \textsc{R}$_x$, \textsc{R}$_y$, $\epsilon>0$)}
 \label{alg:cfr}
\begin{algorithmic}[1]
\STATE $x^{0} =$ uniform strategy at every simplex
\STATE $t = 1$
\WHILE{$\epsilonsad(x^t,y^t)>\epsilon$}
  \STATE $g = -Ay^{t-1}$
  \FORALL{$j \in S_\cX$}
    \STATE $g_{p_j} = g_{p_j} + \langle g^j, \frac{ x^{j,t-1} }{x^{t-1}_{p_j}} \rangle$
    \STATE $x^{j,t} = \textsc{R}_x(g^j)$
  \ENDFOR
  \STATE $\bar{x} = \alpha^t x^t + (1-\alpha^t)\bar{x}$
  \STATE $g = A^Tx^{t}$
  \FORALL{$j \in S_\cY$}
    \STATE $g_{p_j} = g_{p_j} + \langle g^j, \frac{y^{j,t-1}}{y^{t-1}_{p_j}} \rangle$
    \STATE $y^{j,t} = \textsc{R}_y(g^j)$
  \ENDFOR
  \STATE $t=t+1$
  \STATE $\bar{y} = \alpha^t y^t + (1-\alpha^t)\bar{y}$
\ENDWHILE
\STATE \textbf{return} $\bar{x},\bar{y}$
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:rm} shows the regret-minimizer \emph{regret matching} (RM).
Every time RM is called with a gradient vector, it updates the cumulative regret
$r^t$ associated with each action (i.e. how much better that action has
historically been compared to the current strategy). A new strategy is then
computed by setting the probability on each action proportional to the positive
cumulative regret associated with the action ($[\cdot]^+$ denotes the operation
that sets every entry to the maximum of the entry and 0). The average iterate of
RM converges to a strategy with zero regret at a rate of $\frac{1}{\sqrt{T}}$.
\begin{algorithm}[h!]
  \caption{\textsc{RM}($g$)}
 \label{alg:rm}
\begin{algorithmic}[1]
  \STATE // Initial state
  \STATE $r^{0} = 0$
  \STATE $t = 1$
  \FORALL{calls to \rmp}
    \STATE $r^t = r^{t-1} + g - \overrightarrow{1}_n\langle z^{t-1}, g \rangle$
    \STATE $z^t = \frac{[r^{t}]^+}{\|[r^{t}]^+\|_1}$ // if $r^{t}=0$ use uniform strategy
    \STATE $t = t+1$
  \ENDFOR
\STATE \textbf{return} $z^t$
% \ENDPROCEDURE
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:rmp} shows the regret-minimizer \emph{regret matching plus}
(\rmp). {\rmp} works the same as RM except that the cumulative regret is
thresholded at zero at every iteration (thus negative regret never accumulates).
While {\rmp} converges at the same rate as RM in theory, it has been observed to
work better in practice~\citep{Tammelin15:Solving}.
\begin{algorithm}[h!]
  \caption{\textsc{\rmp}($g$)}
 \label{alg:rmp}
\begin{algorithmic}[1]
  \STATE // Initial state
  \STATE $r^{0} = 0$
  \STATE $t = 1$
  \FORALL{calls to \rmp}
    \STATE $r^t = [r^{t-1} + g - \overrightarrow{1}_n\langle z^{t-1}, g \rangle]^+$
    \STATE $z^t = \frac{r^{t}}{\|r^{t}\|_1}$ // if $r^{t}=0$ use uniform strategy
    \STATE $t = t+1$
  \ENDFOR
\STATE \textbf{return} $z^t$
% \ENDPROCEDURE
\end{algorithmic}
\end{algorithm}

CFR(RM) uses a stepsize sequence $\alpha^t=\frac{1}{t}$ for all $t$ and the RM
regret minimizer. CFR({\rmp}) also uses $\alpha^t=\frac{1}{t}$ for all $t$ but
the {\rmp} regret minimizer. Finally {\cfrp} uses stepsizes $\alpha^t =
\frac{2t}{t^2+t}$ and the {\rmp} regret minimizer. \citet{Tammelin15:Solving}
showed that the choice of stepsize in {\cfrp} converges with {\rmp}, but not
with RM.

{\cfrp} has a proven theoretical convergence rate that is proportional to
$1/\sqrt{T}$: \citet{Tammelin15:Solving} show that after $T$ iterations of
{\cfrp}, the maximum regret for Player $1$ is upper bounded by (a similar bound
holds for Player $2$)
  \[
    2 |S_\cX| L \frac{\sqrt{\max \{|\Delta_j| : j \in S_\cX\}}}{\sqrt{T}},
  \]
  where $L$ is the maximum payoff difference for Player $1$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../ijcai18/gpu_egt_river_ijcai18"
%%% End:

